gaBERT -- an Irish Language Model

The BERT family of neural language models have become highly popular due to their ability to provide sequences of text with rich context-sensitive token encodings which are able to generalise well to many NLP tasks. We introduce gaBERT, a monolingual BERT model for the Irish language. We compare our gaBERT model to multilingual BERT and the monolingual Irish WikiBERT, and we show that gaBERT provides better representations for a downstream parsing task. We also show how different filtering criteria, vocabulary size and the choice of subword tokenisation model affect downstream performance. We compare the results of fine-tuning a gaBERT model with an mBERT model for the task of identifying verbal multiword expressions, and show that the fine-tuned gaBERT model also performs better at this task. We release gaBERT and related code to the community.

==> abstract.tex <==

The BERT family of neural language models have become highly popular due to their ability to provide sequences of text with rich
context-sensitive token encodings which are able to generalise well to many NLP tasks.
We introduce, gaBERT, a monolingual BERT model for the Irish language.
We compare our gaBERT model to
multilingual BERT and monolingual WikiBERT,
and we
show that gaBERT provides better representations for a downstream parsing task.
We also show
how
different filtering criteria,
vocabulary size
and the choice of subword tokenisation model
affect downstream performance.
We release gaBERT and related code to the community.

\\ \newline \Keywords{BERT, Irish} 

==> appendices/more-future-work.tex <==
% appendix: more future work ideas

The following list of future work ideas has been collected from our
GitHub repository. \NOTE{Issue numbers refer to this repository.}
\begin{itemize}
    \item Effect of switching to v8 of Paracrawl \NOTE{issue \#77}
    \item Effect of random initialisation (using the same model type and settings as in the development phase; purpose is to find out whether the observed differences between settings are meaningful; differences that can be explained with model instability and that contradict expectations can then be disregarded)
    \item For each corpus, effect of removing it
    \item For each pair of corpora, effect of removing them
    \item Start with the NCI and add corpora in order of cleanliness (or data value estimate from above corpus ablation)
    \item More on filter thresholds and/or corpus-specific filter settings \NOTE{issue \#72}
    \item Effect of filtering (near) duplicates \NOTE{issue \#73}
    \item Effect of increasing the weight of clean corpora \NOTE{issue \#53}
    \item Restrict vocabulary building to clean corpora \NOTE{issue \#54}
    \item Partition the corpus, create a vocabulary for each partition and join the vocabularies \NOTE{issue \#33}
    \item Effect of \#\# glue on prefixes \NOTE{issue \#80}
    \item Effect of adding our in-house Irish Twitter corpora, in particular on tasks involving social media content \NOTE{issue \#34}
    \item Add a copy of the data with accents removed and/or other normalisations \NOTE{issue \#30}
    \item Add synthetic Irish, \eg MT output \NOTE{issue \#14}
    \item Add Hiberno-English corpora and English side of parallel corpora to training data \NOTE{issue \#13}
    \item The role of sentence-splitting, \eg does BERT need to see properly formed sentences or are snippets of text sufficient?
\end{itemize}

==> appendices/reproducibility-checklist.tex <==


\NOTE{We probably will have to complete the following checklist. Let's keep this here as a reminder.}
%
For all reported experimental results:
\begin{itemize}
    \item A clear description of the mathematical setting, algorithm, and/or model
    \item A link to a downloadable source code, with specification of all dependencies, including external libraries (recommended for camera ready, though welcome for initial submission)
    \TODO{Is this for the final version?
    Shouldn't this go into a supplement zip file in the submission?}
    \item A description of computing infrastructure used
    \item The average runtime for each model or algorithm, or estimated energy cost
    \item The number of parameters in each model
    \item Corresponding validation performance for each reported test result    
    \item A clear definition of the specific evaluation measure or statistics used to report results. 
\end{itemize}

\noindent
For all results involving multiple experiments, such as hyperparameter search:
\begin{itemize}
    \item The exact number of training and evaluation runs
    \item The bounds for each hyperparameter
    \item The hyperparameter configurations for best-performing models
    \item The method of choosing hyperparameter values (e.g. manual tuning, uniform sampling, etc.) and the criterion used to select among them (e.g. accuracy)
    \item Summary statistics of the results (e.g. mean, variance, error bars, etc.)
\end{itemize}
    
\noindent
For all datasets used:
\begin{itemize}
    \item Relevant statistics such as number of examples and label distributions
    \item Details of train/validation/test splits
    \item An explanation of any data that were excluded, and all pre-processing steps
    \item For natural language data, the name of the language(s)
    \item A link to a downloadable version of the dataset or simulation environment
    \TODO{Venues that strictly require all used data sets to be publicly available will not
    be suitable for our NCI-based work. What top conferences still are open to us?} 
\end{itemize}
